On the Complexity of Anonymous Communication Through Public Networks

Onion routing is the most widely used approach to anonymous communication online. The idea is that Alice wraps her message to Bob in layers of encryption to form an "onion," and routes it through a series of intermediaries. Each intermediary's job is to decrypt ("peel") the onion it receives to obtain instructions for where to send it next, and what to send. The intuition is that, by the time it gets to Bob, the onion will have mixed with so many other onions, that its origin will be hard to trace even for an adversary that observes the entire network and controls a fraction of the participants, possibly including Bob. In spite of its widespread use in practice, until now no onion routing protocol was known that simultaneously achieved, in the presence of an active adversary that observes all network traffic and controls a constant fraction of the participants, (a) fault-tolerance, where even if a few of the onions are dropped, the protocol still delivers the rest; (b) reasonable communication and computational complexity as a function of the security parameter and the number of participants; and (c) anonymity. In this paper, we give the first onion routing protocol that meets these goals: our protocol (a) tolerates a polylogarithmic (in the security parameter) number of dropped onions and still delivers the rest; (b) requires a polylogarithmic number of rounds and a polylogarithmic number of onions sent per participant per round; and (c) achieves anonymity. We also show that to achieve anonymity in a fault-tolerant fashion via onion routing, this number of onions and rounds is necessary. Of independent interest, our analysis introduces two new security properties of onion routing -- mixing and equalizing -- and we show that together they imply anonymity.

==> mixing-general.tex <==
\subsection{Mixing for an arbitrary input set} \label{sec:mix2}
In Section~\ref{sec:mix}, we gave the definition of mixing in the simple I/O setting. 
%
Our formal definition, below, extends the definition to any arbitrary input set $\Sigma$: 

\paragraph{The mixing game} 
Let $\mathcal{OE} = (\gen, \formonion, \proconion)$ be a secure onion encryption scheme. 
The mixing game $\mathsf{GeneralMixingGame}(\secparam, \Pi, \adv, \Sigma)$ is parametrized by the security parameter $\secparam$, an onion routing protocol $\Pi$, an adversary $\adv$, and a set $\Sigma$ of input vectors. 

The adversary $\adv$ chooses a subset $\Bad \subseteq \parties$ of the parties to corrupt and also chooses the keys for these parties. Let $\pk(\Bad)$ be a shorthand for the corrupted parties' public keys. 

For each honest party $P\in\parties\setminus\Bad$, $\adv$ assigns a number, $\mathsf{numSends}(P)$, of challenge messages for $P$ to send; the \emph{target senders} are the parties that are instructed to send one or more challenge messages. 
%
For each party $P\in\parties$, $\adv$ also assigns a number, $\mathsf{numReceives}(P)$, of challenge messages for $P$ to receive such that $\sum_{P\in\parties}^N \mathsf{numReceives}(P) = \sum_{P\in\parties\setminus\Bad} \mathsf{numSends}(P)$; the \emph{target recipients} are the recipients of the challenge messages to be sent out by the target senders. 

Let $\senders$ be the \emph{multiset} of target senders so that for every $P\in\parties$, there are $\mathsf{numSends}(P)$ instances of $P$ in $\senders$. Likewise, let $\receivers$ be the \emph{multiset} of target recipients so that for every $P\in\parties$, there are $\mathsf{numReceives}(P)$ instances of $P$ in $\receivers$. 
$\adv$ sends $(\Bad, \pk(\Bad), \senders, \receivers, \tilde\sigma)$ to the challenger $\cdv$. 

Let $\tilde m \in \mathcal{M}$ denote the special challenge message so that every other message $m \in \mathcal{M}$ is distinct from $\tilde m$. 
%
The challenger $\cdv$ supplies the rest of the input vector $\sigma = (\sigma_1, \dots, \sigma_N)$ by choosing a random bijection $g$ from $\senders$ to $\receivers$; each $P_i \in \senders$ is instructed to send the challenge message $\tilde m \in \mathcal{M}$ to $g(P_i) \in \receivers$, i.e., $\{(\tilde m, g(P_i)\} \in \sigma_i$.
If the input vector $\sigma$ is not in $\Sigma$, $\cdv$ keeps trying randomly chosen bijections from $\senders$ to $\receivers$ until she gets an input from $\Sigma$. 
%
Let $\mathsf{numBijections}$ denote the number of bijections that can ``complete'' an input in $\Sigma$ in this way. 

Next, $\cdv$ interacts with $\adv$ in an execution of protocol $\Pi$ on input $\sigma$ with $\cdv$ acting as the honest parties adhering to the protocol and $\adv$ controlling the corrupted parties. Whenever the protocol $\Pi$ specifies for an onion to be formed or processed, $\cdv$ runs the onion encryption scheme's onion-forming algorithm $\formonion$ or onion-processing algorithm $\proconion$.

Let $\mathsf{O}_{\receivers}$ be the set of onions received by the parties in $\receivers$. At the end of the execution, $\adv$ outputs an onion $O \in \mathsf{O}_{\receivers}$ and its guess, a sender $S \in \senders$, of a party one of whose calls to $\formonion$ returned $O$ as one of its onions.

Let an onion be a ``\emph{valid challenge onion}'' if peeling the outermost layer produces the challenge message $\tilde m$. 
If $O$ is a valid challenge onion, $\adv$ wins iff $S$ is the sender of $O$. 
Otherwise if $O$ is not a valid challenge onion, $\adv$ wins with probability $\frac{1}{\mathsf{numBijections}}$. 
%
See Figure~\ref{fig:mix2}. %\todo{Fix the figure.}

\begin{figure}[ht!]
\centering
\procedure{$\mathsf{GeneralMixingGame}(\secparam, \Pi, \adv, \Sigma)$}{%
\adv \> \> \cdv \\
\text{pick } \Bad \subseteq \parties \\ 
\text{pick multiset $\senders$ of target senders} \\
\text{pick multiset $\receivers$, $|\receivers| = |\senders|$ of target receivers} \\
\text{pick the partial input vector } \tilde\sigma \\
\> \sendmessageright*[3.0cm]{\Bad, \pk(\Bad), \senders, \receivers, \tilde\sigma} \\
\> \sendmessageleft*[3.0cm]{\pk(\parties\setminus\Bad)} \\
\> \> \text{randomly pick remaining inputs for } \sigma \pclb
\pcintertext[dotted]{interact in run of protocol $\Pi$ on input $\sigma$} \\
\text{guess and output $O \in \mathsf{O}_{\receivers}$ and $S\in\senders$} \\
}
\caption{Schematic of the general mixing game.}
\label{fig:mix2}
\end{figure}

Let the advantage of the general mixing game be 
\[
\mathsf{AdvGeneralMixingGame}(\secparam, \Pi, \adv, \Sigma) = \left|\prob{\text{$\adv$ wins}} - \frac{1}{\mathsf{numBijections}} \right| . 
\]

We now define mixing as follows. 

\begin{definition} [Mixing for arbitrary input sets] \label{def:mix2}
\sloppy An onion routing protocol $\Pilong$ mixes for the adversary class $\mathbb{A}$ w.r.t.\ the input set $\Sigma$ if for every adversary $\adv \in \mathbb{A}$,  
\[
\mathsf{AdvGeneralMixingGame}(\secparam, \Pi, \adv, \Sigma) = \negl .
\]

The protocol computationally (resp.\ statistically) mixes if the adversaries in $\mathbb{A}$ are computationally bounded (resp.\ unbounded). 
\end{definition} 

==> mixing2.tex <==
\subsection{Mixing  in the simple I/O setting} \label{sec:mix}
Mixing is a property of \emph{onion routing} protocols. 
Informally, an onion routing protocol mixes if the protocol sufficiently shuffles the honest parties' ``message-bearing'' onions. That is, once an honestly generated onion has traveled far enough, getting peeled at every intermediary, the adversary cannot trace it to the original sender.  If the adversary is the recipient of the message contained in the onion, it should not be able to trace it to the sender provided the message itself does not reveal the sender.

Formally, mixing is defined with respect to the mixing game. To keep things simple, we present the definition in the simple I/O setting. This can be extended for any arbitrary input set; see \emph{Supplementary materials} for the general definition of mixing over any arbitrary input set.

\paragraph{The mixing game} 
Let $\mathcal{OE} = (\gen, \formonion, \proconion)$ be a secure onion encryption scheme. 
The mixing game $\mathsf{MixingGame}(\secparam, \Pi, \adv)$ is parametrized by the security parameter $\secparam$, an onion routing protocol $\Pi$, and an adversary $\adv$. 

The adversary $\adv$ chooses a subset $\Bad \subseteq \parties$ of the parties to corrupt and also chooses the keys for these parties. Let $\pk(\Bad)$ be a shorthand for the corrupted parties' public keys. 
$\adv$ also identifies a set $\senders \subseteq \parties \setminus \Bad$ of honest \emph{target senders} and a set $\receivers \subseteq \parties$, $|\receivers| = |\senders|$ of \emph{target receivers}. 

\iffalse
\todo{move to a less prominent place} For any sequence $\tilde\tau = (\tilde\tau_1, \tilde\tau_2, \dots, \tilde\tau_N)$ of sets of message-receiver pairs and for any bijection~$f$ from a set $A\subseteq\parties$ of parties to a set $B\subseteq\parties$ of parties, let $\tilde \tau \sqcup f \myeq (\tau_1, \tau_2, \dots, \tau_N)$ where 
$\tau_i = \tilde\tau_i \cup \{(\tilde m, f(P_i))\}$ for every $P_i \in A$ and 
$\tau_i = \tilde\tau_i$ for every $P_i \not\in A$. 

Let a sequence $\tilde\sigma = (\tilde\sigma_1, \tilde\sigma_2, \dots, \tilde\sigma_N)$ of sets of message-receiver pairs be a ``\emph{partial input vector for senders $\senders$ and receivers $\receivers$}'' if for any bijection $g : \senders \mapsto \receivers$ mapping from $\senders$ to $\receivers$,
the sequence $\sigma = \tilde\sigma \sqcup g$ is in the input set $\Sigma$. 

Finally, for a partial input vector $\tilde\sigma$ for $\senders$ and $\receivers$, let $\Sigma_{\tilde\sigma}^{\senders, \receivers}$ be the set of all input vectors $\sigma = \tilde\sigma \sqcup g$ where $g$ is a bijection from $\senders$ to $\receivers$. 
\todo{end(move)}
\fi

In addition to $\Bad$, $\pk(\Bad)$, $\senders$, and $\receivers$, 
$\adv$ also decides \emph{part} of the input; for every non-target sender $P_i \in \parties\setminus\senders$, $\adv$ chooses a message $m$ and a unique non-target recipient $P_j \in\parties\setminus\receivers$ such that $P_i$'s input becomes $\sigma_i = \{(m, P_j)\}$. We call this collection of inputs that $\adv$ decides ``\emph{the partial input vector},'' and denote it $\tilde \sigma$.   \todo{would get stronger security if $\tilde{\sigma}$ were chosen after adversary has seen the public keys.}
%
$\adv$ sends $(\Bad, \pk(\Bad), \senders, \receivers, \tilde\sigma)$ to the challenger $\cdv$.

For each honest party in $\parties\setminus\Bad$, $\cdv$ generates a key pair for the party by running the onion encryption scheme's key generating algorithm $\gen$ and sends the public keys $\pk(\parties\setminus\Bad)$ of the honest parties to the adversary~$\adv$. 

Let $\tilde m \in \mathcal{M}$ denote the special challenge message so that every other message $m \in \mathcal{M}$ is distinct from $\tilde m$. 
The challenger $\cdv$ supplies the rest of the input vector $\sigma = (\sigma_1, \dots, \sigma_N)$ by choosing a random bijection $g$ from $\senders$ to $\receivers$; each $P_i \in \senders$ is instructed to send the challenge message $\tilde m \in \mathcal{M}$ to $g(P_i) \in \receivers$, i.e., $\sigma_i = \{(\tilde m, g(P_i)\}$. 

\iffalse
Next, the challenger $\cdv$ picks destinations for the messages sent by the targeted honest senders. Let the set $\sample \Sigma_{\tilde\sigma}^{\senders, \receivers}$ be \todo{define}.  $\cdv$ generates a random $\sigma\leftarrow \Sigma_{\tilde\sigma}^{\senders, \receivers}$.
\fi

Next, $\cdv$ interacts with $\adv$ in an execution of protocol $\Pi$ on input $\sigma$ with $\cdv$ acting as the honest parties adhering to the protocol and $\adv$ controlling the corrupted parties. Whenever the protocol $\Pi$ specifies for an onion to be formed or processed, $\cdv$ runs the onion encryption scheme's onion-forming algorithm $\formonion$ or onion-processing algorithm $\proconion$.

Let $\mathsf{O}_{\receivers}$ be the set of onions received by the parties in $\receivers$. At the end of the execution, $\adv$ outputs an onion $O \in \mathsf{O}_{\receivers}$ and its guess, a sender $S \in \senders$, of a party one of whose calls to $\formonion$ returned $O$ as one of its onions.

Let an onion be a ``\emph{valid challenge onion}'' if peeling the outermost layer produces the challenge message $\tilde m$. 
If $O$ is a valid challenge onion, $\adv$ wins iff $S$ is the sender of $O$. 
Otherwise if $O$ is not a valid challenge onion, $\adv$ wins with probability $\frac{1}{|\senders|}$. 
%
See Figure~\ref{fig:mix}. 

\begin{figure}[ht!]
\centering
\procedure{$\mathsf{MixingGame}(\secparam, \Pi, \adv)$}{%
\adv \> \> \cdv \\
\text{pick } \Bad \subseteq \parties \\ 
\text{pick honest target senders } \senders \subseteq \parties \setminus \Bad \\
\text{pick target receivers } \receivers \subseteq \parties \text{ s.t. } |\receivers| = |\senders| \\
\text{pick the partial input vector } \tilde\sigma \\
\> \sendmessageright*[3.0cm]{\Bad, \pk(\Bad), \senders, \receivers, \tilde\sigma} \\
\> \sendmessageleft*[3.0cm]{\pk(\parties\setminus\Bad)} \\
\> \> \text{randomly pick remaining inputs for } \sigma \pclb
\pcintertext[dotted]{interact in run of protocol $\Pi$ on input $\sigma$} \\
\text{guess and output $O \in \mathsf{O}_{\receivers}$ and $S\in\senders$} \\
}
\caption{Schematic of the mixing game.}
\label{fig:mix}
\end{figure}

Let the advantage of the mixing game be 
\[
\mathsf{AdvMixingGame}(\secparam, \Pi, \adv) = \left|\prob{\text{$\adv$ wins}} - \frac{1}{|\senders|} \right| . 
\]

We now define mixing as follows. 

\begin{definition} [Mixing] \label{def:mix}
\sloppy An onion routing protocol $\Pilong$ mixes for the adversary class $\mathbb{A}$ in the simple I/O setting if for every adversary $\adv \in \mathbb{A}$,  
\[
\mathsf{AdvMixingGame}(\secparam, \Pi, \adv) = \negl .
\]

The protocol computationally (resp.\ statistically) mixes if the adversaries in $\mathbb{A}$ are computationally bounded (resp.\ unbounded). 
\end{definition} 

%\todo{A paragraph on intuition}
Now that we have defined mixing formally, let us walk the reader through our definitional choices.  The starting intuition that this definition needs to capture is that it should be hard for the adversary to pinpoint the origin of an onion received by one of the target recipients.  Thus, the adversary's probability of identifying the origin of an onion should be close to $1/|\senders|$.

This goal comes with a caveat that of course an adversary can determine the sender of an onion that one of the targeted senders has just created, or, more generally, that hasn't traveled very far and hasn't had a chance to mix with any onions from other target senders.  Hence, we need to restrict the set of onions on which the adversary can win to a set of onions that have traveled far and have already had a chance to mix with other onions.  This is why we have the (admittedly somewhat artificial) requirement that the onion be a valid challenge onion, i.e. that, when peeled, it yields the special message $\tilde{m}$.

A problem with this definition of a valid challenge onion is that, if the onion's recipient is honest, then the adversary should not necessarily be able to determine whether a particular onion is a valid challenge onion or not, and we don't want the mere fact that the adversary won or lost the game to give him information.  Thus, should the adversary pick an onion that is not a valid challenge onion, the security game still allows him to win with probability $1/|\senders|$.  

\iffalse
\begin{remark}
In general, anonymity does not mixing. Consider the simple protocol in which everyone sends an onion to everyone; for all but the intended recipient the onion is a dummy one.  This protocol is anonymous for the network adversary even though it does not mix.
\end{remark}
\fi

==> thmimpliedby.tex <==
\begin{proof}
Let $\sigma$ and $\sigma'$ be \emph{swap-neighboring} if there exist parties $i, j \in \parties$, such that (i) $\sigma_k = \sigma'_k$ for every party $k \notin \{i, j\}$, (ii) $\sigma_i = \sigma'_j$ and (iii) $\sigma_j = \sigma'_i$. 

Consider a variant of the anonymity game in which the adversary always chooses swap-neighboring input vectors for the challenge input vectors $\sigma^0$ and $\sigma^1$. 
%
It can be shown that 

\begin{claim}
The OR protocol $\Pi$ anonymizes from the adversary class $\mathbb{A}$  w.r.t.\ the input set $\Sigma$ iff every adversary $\adv \in \mathbb{A}$ wins the variant of the anonymity game with negligible advantage. (The reader can easily check this claim.) 
\end{claim}

To prove the theorem, we assume that $\Pi$ equalizes and construct a reduction~$\bdv$ that wins the mixing game $\mathsf{MixingGame}(\secparam, \Pi, \adv, \Sigma, \mathsf{all})$ with nonnegligible advantage from an adversary $\adv$ that wins the variant of the anonymity game with nonnegligible advantage. 

\begin{enumerate}
\item Let $\Bad$, $\pk(\Bad)$, and $\sigma^0$ and $\sigma^1 = \mathsf{swap}(\sigma^0, i, j)$ be the adversary $\adv$'s choices for the set of corrupted parties, the public keys for the corrupted parties, and the swap-neighboring challenge input vectors. 
%
%The reduction~$\bdv$ chooses new keys for the corrupted parties in $\Bad$. 

\item Let $r^0_i$ be the receiver of $i$ in $\sigma^0$, and let $r^0_j$ be the receiver of $j$ in $\sigma^0$. 
Let $\senders = \{i, j\}$ and let $\receivers = \{r^0_i, r^0_j\}$. 
$\bdv$ determines the partial input vector $\tilde\sigma$ such that $\Sigma_{\tilde\sigma}^{\senders, \receivers} = \{\sigma^0, \sigma^1\}$ and sends $\Bad$, $\pk(\Bad)$, $\senders$, $\receivers$ and $\tilde\sigma$ to the challenger $\cdv$.  

\item The challenger $\cdv$ and the adversaries $\adv$ and $\bdv$ interact in an execution of protocol $\Pi$ on input $\sigma \sample \Sigma_{\tilde\sigma}$ (sampled and kept secret by $\cdv$) with $\cdv$ acting as the honest parties adhering to the protocol and $\adv$ (via $\bdv$) controlling the corrupted parties. %(At every round, $\bdv$ creates the view so far for $\adv$ by decrypting all onion layers that can be decrypted using the corrupted parties secret keys $\sk(\Bad, \bdv)$ and redoing the encryptions using the public keys $\pk(\Bad, \adv)$.)

\item Let $\mathcal{O}^0_i$ be the set of honest onions received by $r^0_i$, and 
let $\mathcal{O}^0_j$ be the set of honest onions received by $r^0_j$. 
%
At the end of the execution, $\bdv$ picks a random onion $o^0 \sample \mathcal{O}^0_i$ from $ \mathcal{O}^0_i$ and a random onion $o^1 \sample \mathcal{O}^0_j$ from $\mathcal{O}^0_j$ and sends $(o^0, o^1)$ to $\cdv$. 

\item Upon receiving the identity $s$ of a sender from $\cdv$ and 
a guess~$b'$ from $\adv$,  
$\bdv$ computes his guess $b''$ (for which onion was chosen by $\cdv$) as follows: 
\begin{enumerate}
\item If $b' = 0$ and $s = i$, then $\bdv$ outputs $b'' = 0$. He guesses that the challenger chose the onion $o^0 \in \mathcal{O}^0_i$ received by receiver $r^0_i$. 

\item If $b' = 0$ and $s = j$, then $\bdv$ outputs $b'' = 1$. He guesses that the challenger chose $o^1 \in \mathcal{O}^0_j$ received by $r^0_j$. 

\item If $b' = 1$ and $s = i$, then $\bdv$ outputs $b'' = 1$. He guesses that the challenger chose $o^1 \in \mathcal{O}^0_j$ received by $r^0_j$ (who is also the receiver of $i$ in $\sigma^1$). 

\item If $b' = 1$ and $s = j$, then $\bdv$ outputs $b'' = 0$. He guesses that the challenger chose $o^0 \in \mathcal{O}^0_i$ received by $r^0_i$ (who is also the receiver of $j$ in $\sigma^1$). 
\end{enumerate}
\end{enumerate}

When $\Pi$ is indifferent and equalizes, the adversaries' view on input $\sigma^0$ is indistinguishable from that on input $\sigma^1$. Thus, if $\adv$ can distinguish a protocol run on input $\sigma^0$ from a run on input $\sigma^1$, it implies that $\Pi$ does not mix. 
\end{proof}

